Approximating the minimum cycle mean

We consider directed graphs where each edge is labeled with an integer weight and study the fundamental algorithmic question of computing the value of a cycle with minimum mean weight. Our contributions are twofold: (1) First we show that the algorithmic question is reducible in O(n^2) time to the problem of a logarithmic number of min-plus matrix multiplications of n-by-n matrices, where n is the number of vertices of the graph. (2) Second, when the weights are nonnegative, we present the first (1 + {\epsilon})-approximation algorithm for the problem and the running time of our algorithm is \tilde(O)(n^\omega log^3(nW/{\epsilon}) / {\epsilon}), where O(n^\omega) is the time required for the classic n-by-n matrix multiplication and W is the maximum value of the weights.

==> eptcsdata.tex <==
\providecommand{\firstpage}{136}
\providecommand{\publicationstatus}{Gabriele Puppis, Tiziano Villa (Eds.): Fourth International\\ Symposium on Games, Automata, Logics and Formal Verification\\
EPTCS 119, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.119.13}{10.4204/EPTCS.119.13}}

